Alternating Objectives Generates Stronger PGD-Based Adversarial Attacks

Designing powerful adversarial attacks is of paramount importance for the evaluation of $\ell_p$-bounded adversarial defenses. Projected Gradient Descent (PGD) is one of the most effective and conceptually simple algorithms to generate such adversaries. The search space of PGD is dictated by the steepest ascent directions of an objective. Despite the plethora of objective function choices, there is no universally superior option and robustness overestimation may arise from ill-suited objective selection. Driven by this observation, we postulate that the combination of different objectives through a simple loss alternating scheme renders PGD more robust towards design choices. We experimentally verify this assertion on a synthetic-data example and by evaluating our proposed method across 25 different $\ell_{\infty}$-robust models and 3 datasets. The performance improvement is consistent, when compared to the single loss counterparts. In the CIFAR-10 dataset, our strongest adversarial attack outperforms all of the white-box components of AutoAttack (AA) ensemble, as well as the most powerful attacks existing on the literature, achieving state-of-the-art results in the computational budget of our study ($T=100$, no restarts).

==> algorithms/PGD.tex <==
\begin{algorithm*}
  \small
  \caption{White-box PGD-based attack (Adapted from \cite{Gowal2019AnAS})}
  \begin{algorithmic}[1]
    \Statex \textbullet~\textbf{Input:} A nominal input $x$ and label $y$, a model $f_{\theta}$ and an adversarial set $\Delta(x)$. $\alpha^{(k)}$ is the step-size at iteration $k$ and \texttt{Opt} is an optimizer (e.g., Adam).
    \Statex \textbullet~\textbf{Output:} Possible attack $\hat{\xi} \in \Delta(x)$.
    \State $\widehat{\xi} \leftarrow x $ 
    \For{$r \in \{1,...,R\}$} \Comment{Repeat the attack process $R$ times}
        \State \text{Initialize surrogate loss} $\hat{L}^{(r)}$ \Comment{The surrogate loss may be different across restarts}
        \State \text{Initialize optimizer \texttt{Opt}} \Comment{The optimizer ingests gradients and computes an update}
        \State $\xi^{(0)} \gets \texttt{SampleFrom}(x,\Delta)$
        \For{$k \in \{1,...,K\}$} \Comment{$K$ corresponds to the number of optimization steps}
            \State  $\xi^{(k)} \gets \texttt{Proj}_{\Delta(x)} \Big ( \xi^{(k-1)} + \alpha^{(k)} \texttt{Opt} \big ( \nabla_{ \xi^{(k-1)}} \hat{L}^{(r)}(f_{\theta}( \xi^{(k-1)}),y) \big ) \Big ) $
            \If{$L(f_{\theta}(\xi^{(k)}),y) > L(f_{\theta}(\xi),y)$} \Comment{$L$ is the loss of interest (e.g., 0-1 loss)}
                \State $\hat{\xi} \gets \xi^{(k)}$ \Comment{If $L$ is the 0-1 loss, the procedure can terminate early}
            \EndIf
        \EndFor
    \EndFor
  \end{algorithmic}
\end{algorithm*}

==> tables/autoattack.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{r  c c c >{\bfseries}c}
    \toprule
    Model ID & $\apgdce$ & $\apgddlr$ & FAB & \normalfont{$\cecwdlr$}  \\ 
    \cmidrule(lr){1-1}  \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule{5-5}
    Engstrom2019Robustness \cite{robustness}       & 51.72 & 52.67 & 50.67 & 50.27 \\
    Carmon2019Unlabeled \cite{carmon2019unlabeled} & 61.74 & 60.67 & 60.88 & 59.97\\
    Hendrycks2019Using \cite{hendrycks2019using}  & 57.23 & 57.03 & 55.55 & 55.35 \\
    Zhang2019You \cite{zhang2019you}              & 46.15 & 47.39 & 45.83 & 45.32 \\
    Zhang2019Theoretically \cite{zhang2019theoretically} \dag      & 55.28 & 53.52 & 53.92 & 53.41 \\
    Wu2020Adversarial \cite{wu2020adversarial}  & 58.90 & 56.68 & 56.82 & 56.42 \\
    Sehwag2021Proxy\_R18\cite{sehwag2021robust} & 58.38 & 57.37 & 56.27 & 56.06 \\
    Andriushchenko2020Understanding \cite{andriushchenko2020understanding}  & 46.93 & 47.08 & 44.72 & 44.50 \\
    Dai2021Parameterizing \cite{dai2021parameterizing}               & 63.93 & 63.44 & 62.27 & 61.77\\
    Gowal2021Improving\_28\_10\_ddpm\_100m\cite{gowal2021improving}  & 65.63 & 65.14 & 64.14 & 63.84 \\
    Huang2021Exploring\_ema \cite{huang2021exploring}        & 64.55 & 64.14 & 64.45 & 63.06 \\
    Zhang2020Geometry \cite{zhang2020geometry}               & 66.37 & 60.19 & 59.97 & 59.69 \\
    Rade2021Helper\_R18\_extra \cite{rade2021helperbased}    & 61.40 & 58.41 & 58.42 & 57.74 \\
    Addepalli2021Towards\_RN18 \cite{addepalli2021towards}   & 55.80 & 51.56 & 51.93 & 51.41 \\
    Sehwag2020Hydra \cite{sehwag2020hydra}                   & 59.60 & 58.29 & 58.29 & 57.61 \\
    \bottomrule
    \end{tabular}
\vspace{0.2cm}
\caption{Comparing $\cecwdlr$ with the untargeted version of every single white-box component from the AutoAttack ensemble. The experiments are executed for $T=100$ with no restarts. Each entry reports the robust accuracy of each classifier for the given method. (\dag): Attacked with $\epsilon=0.031$.}
\label{table:autoattack}
\end{table*}

==> tables/baselines.tex <==
\begin{table*}[!ht]
\centering
\hspace*{-1cm}
\begin{tabular}{r c c c |  c c c}
    \toprule
    Model ID & $\cecwdlr$  & GAMA-PGD \cite{Sriramanan2020GuidedAA} & $\Delta$  & $\cecwdlr$  & MD Attack \cite{Ma2020ImbalancedGA} & $\Delta$\\
          & (GAMA-PGD sch.)  &                                   &           & (MD sched.)   & &    \\
    \midrule
    Engstrom2019Robustness~\cite{robustness}       & \textbf{49.88} & 50.05          & -0.17 & \textbf{49.87} & 50.34 & -0.47\\
    Carmon2019Unlabeled~\cite{carmon2019unlabeled} & \textbf{59.78} & 59.84          & -0.06 & \textbf{59.72} & 59.83 & -0.11\\
    Hendrycks2019Using~\cite{hendrycks2019using}   & 55.26          & \textbf{55.22} & +0.04 & 55.20 & \textbf{55.15} & +0.05\\
    Zhang2019You~\cite{zhang2019you}               & \textbf{45.20} & 45.32          & -0.12 & \textbf{45.17} & 45.49 & -0.32\\
    Zhang2019Theoretically~\cite{zhang2019theoretically}\dag & 53.29          & 53.29          & 0     & \textbf{53.26} & 53.36 & -0.10 \\
    Wu2020Adversarial~\cite{wu2020adversarial}               & 56.30          & 56.30          & 0     & \textbf{56.26} & 56.28 & -0.02\\
    Sehwag2021Proxy\_R18~\cite{sehwag2021robust}              & \textbf{55.95} & 56.01          & -0.06 & \textbf{55.89} & 55.92 & -0.03\\
    Andriushchenko2020Understanding~\cite{andriushchenko2020understanding}  & \textbf{44.41} & 44.42   & -0.01 & \textbf{44.44} & 44.57 & -0.13\\
    Dai2021Parameterizing~\cite{dai2021parameterizing}            & \textbf{61.74} & 61.94          & -0.20 & \textbf{61.72} & 61.99 & -0.27\\
    Gowal2021Improving\_28\_10\_ddpm\_100m~\cite{gowal2021improving}  & \textbf{63.72} & 63.78          & -0.06 & \textbf{63.73} & 63.94 & -0.21\\
    Huang2021Exploring\_ema~\cite{huang2021exploring}              & 62.89          & \textbf{62.87} & +0.02 & \textbf{62.86} & 62.93 & -0.07\\
    Zhang2020Geometry~\cite{zhang2020geometry}                    & \textbf{59.62} & 60.72          & -1.10 & \textbf{59.58} & 59.73 & -0.15\\
    Rade2021Helper\_R18\_extra~\cite{rade2021helperbased}           & \textbf{57.73} & 57.78          & -0.05 & \textbf{57.72} & 57.74 & -0.02\\
    Addepalli2021Towards\_RN18~\cite{addepalli2021towards}         & \textbf{51.26} & 51.43          & -0.17 & \textbf{51.25} & 51.30 & -0.05\\
    Sehwag2020Hydra~\cite{sehwag2020hydra}                        & \textbf{57.43} & 57.49          & -0.06 & 57.45 & \textbf{57.31} & +0.14\\
    \bottomrule
    \end{tabular}
\vspace{0.2cm}
\caption{Comparing $\cecwdlr$ with the strongest attacks of our computational budget ($T=100$ with no restarts). $\Delta$ columns report the robust accuracy gap between the compared methods. Each entry reports the robust accuracy of each classifier for the given method. (\dag): Attacked with $\epsilon=0.031$. }
\label{table:baselines}
\end{table*}

==> tables/cifar100.tex <==
\begin{table*}[t]
%\footnotesize
%\scriptsize
\centering
\begin{tabular}{rccccccc}
    \toprule
     & \multicolumn{3}{c}{\emph{K=1}} & \multicolumn{3}{c}{\emph{K=2}} & \emph{K=3} \\
     \\ 
    Model ID & $\ce$ & $\cw$ & $\dlr$ &  $\cecw$ & $\cedlr$ & $\cwdlr$ & $\cecwdlr$ \\ 
    \cmidrule(lr){1-1}  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8}
    
    Rade2021Helper\_R18\_ddpm    & 32.60 & 29.66 & 29.69  & 29.12\fn{-0.54} & 29.08\fn{-0.61}  & 29.66\fn{0}     & 29.12\fn{-0.54}  \\
    Rebuffi2021Fixing\_R18\_ddpm & 31.82 & 29.20 & 29.25  & 28.68\fn{-0.52} & 28.65\fn{-0.60}  & 29.20\fn{0}     & 28.68\fn{-0.52}  \\
    Addepalli2021Towards\_PARN18 & 32.90 & 28.10 & 28.23  & 27.68\fn{-0.42} & 27.63\fn{-0.60}  & 28.10\fn{0}     & 27.67\fn{-0.43}  \\ %AA:27.14
    Rice2020Overfitting          & 20.89 & 20.42 & 20.62  & 19.33\fn{-1.09} & 19.33\fn{-1.29}  & 20.42\fn{0}     & 19.32\fn{-1.10}  \\ %AA:18.95
    Hendrycks2019Using           & 33.17 & 30.84 & 32.34  & 29.43\fn{-1.41} & 29.43\fn{-2.91}  & 30.83\fn{-0.01} & 29.36\fn{-1.48}  \\ %AA:28.42
    Rebuffi2021Fixing\_28\_10\_cutmix\_ddpm & 35.74 & 33.60 & 33.67 & 32.53\fn{-1.07} & 32.50\fn{-1.17} & 33.60\fn{0} & 32.53\fn{-1.07} \\  
    \bottomrule
    \end{tabular}
\vspace{0.2cm}
\caption{(CIFAR100) Comparing single-loss PGD with the multi-stage variant of PGD (with $K=2,3$). PGD starts from the clean point (no added noise). The experiments are executed for $T=100$ with no restarts. Each entry reports the robust accuracy of each classifier for the given method. (\dag): Attacked with $\epsilon=0.031$.}
\label{table:t100its}
\end{table*}

==> tables/imagenet.tex <==
\begin{table*}[t]
%\footnotesize
%\scriptsize
\centering
\begin{tabular}{rccccccc}
    \toprule
     & \multicolumn{3}{c}{\emph{K=1}} & \multicolumn{3}{c}{\emph{K=2}} & \emph{K=3} \\
     \\ 
    Model ID & $\ce$ & $\cw$ & $\dlr$ &  $\cecw$ & $\cedlr$ & $\cwdlr$ & $\cecwdlr$ \\ 
    \cmidrule(lr){1-1}  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8}
    
    Salman2020Do\_R18      & 29.50 & 27.32 & 27.60 & 25.64\fn{-1.68} & 25.62\fn{-1.98} & 27.32\fn{0} & 25.66    \\  % AA : 25.32 
    Salman2020Do\_R50      & 38.78 & 37.62 & 38.04 & 35.30\fn{-2.32} & 35.26           & 37.24       & 35.26    \\  % AA : 34.96       
    Engstrom2019Robustness & 32.64 & 32.64 & 33.16 & 30.00\fn{-2.64} & 29.94           & 32.66       & 29.96    \\  % AA : 29.22
    Wong2020Fast           & 27.50 & 27.46 & 27.86 & 25.76\fn{-1.70} & 25.74           & 27.48       & 25.74        % AA : 26.24 
    \bottomrule
    \end{tabular}
\vspace{0.2cm}
\caption{(ImageNet) Comparing single-loss PGD with the multi-stage variant of PGD (with $K=2,3$). PGD starts from the clean point (no added noise). The experiments are executed for $T=100$ with no restarts. Each entry reports the robust accuracy of each classifier for the given method. (\dag): Attacked with $\epsilon=0.031$.}
\label{table:t100its}
\end{table*}

==> tables/model_collection_v2.tex <==
\begin{table*}[t]
%\footnotesize
    \centering
    \begin{tabular}{c c c c c}
    \toprule 
    \# & Paper & Model ID in \href{https://github.com/RobustBench/robustbench}{RobustBench leaderboard} & Architecture & Standard Acc. (\%) \\
    \midrule 
    1&\cite{robustness}             & Engstrom2019Robustness & ResNet-50 & 87.03\\
    2&\cite{carmon2019unlabeled}    & Carmon2019Unlabeled    & WideResNet-28-10 & 89.69 \\
    3&\cite{hendrycks2019using}     & Hendrycks2019Using     & WideResNet-28-10 & 87.11 \\
    4&\cite{zhang2019you}           & Zhang2019You           & WideResNet-34-10 & 87.20  \\
    5&\cite{zhang2019theoretically} & Zhang2019Theoretically & WideResNet-34-10 & 84.92 \\
    6&\cite{wu2020adversarial}      & Wu2020Adversarial      & WideResNet-34-10 & 85.36 \\
    7&\cite{sehwag2021robust}       & Sehwag2021Proxy\_R18   & ResNet-18 & 84.59\\
    8&\cite{andriushchenko2020understanding} & Andriushchenko2020Understanding & PreActResNet-18  & 79.84 \\
    9&\cite{dai2021parameterizing} & Dai2021Parameterizing                     & WideResNet-28-10 & 87.02 \\
    10&\cite{gowal2021improving}   & Gowal2021Improving\_28\_10\_ddpm\_100m    & WideResNet-28-10 & 87.50\\
    11&\cite{huang2021exploring}   & Huang2021Exploring\_ema    & WideResNet-34-R & 91.23 \\
    12&\cite{zhang2020geometry}    & Zhang2020Geometry          & WideResNet-28-10 & 89.36 \\
    13&\cite{rade2021helperbased}  & Rade2021Helper\_R18\_extra & PreActResNet-18 & 89.02 \\
    14&\cite{addepalli2021towards} & Addepalli2021Towards\_RN18 & ResNet-18 & 80.24  \\
    15&\cite{sehwag2020hydra}      & Sehwag2020Hydra            & WideResNet-28-10 & 88.98 \\  
    %\midrule 
    \bottomrule
    \end{tabular}
    \vspace{0.2cm}
    \caption{Our model collection, consisting of 15 $\linf$-bounded classifiers obtained from the ModelZoo of RobustBench.}
    %\caption{The correspondence between paper citations and ModelIDs (according to RobustBench) that we used in our experiments}
    \label{table:correspondence}
\end{table*}


==> tables/t100its_nocolors.tex <==
\begin{table*}[t]
%\footnotesize
%\scriptsize
\centering
\begin{tabular}{rccccccc}
    \toprule
     & \multicolumn{3}{c}{\emph{K=1}} & \multicolumn{3}{c}{\emph{K=2}} & \emph{K=3} \\
     \\ 
    Model ID & $\ce$ & $\cw$ & $\dlr$ &  $\cecw$ & $\cedlr$ & $\cwdlr$ & $\cecwdlr$ \\ 
    \cmidrule(lr){1-1}  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8}
    
    Engstrom2019Robustness \cite{robustness}          & 52.24 & 52.59 & 53.55 & 50.29 & \textbf{50.22} & 52.63 & 50.27     \\
    Carmon2019Unlabeled \cite{carmon2019unlabeled}    & 62.09 & 60.86 & 61.16 & 60.00 & 60.00    & 60.88 & \textbf{59.97}  \\
    Hendrycks2019Using \cite{hendrycks2019using}      & 57.38 & 56.61 & 57.47 & 55.41 & 55.37          & 56.55 & \textbf{55.35} \\
    Zhang2019You \cite{zhang2019you}                  & 46.28 & 47.44 & 47.97 & 45.33 & \textbf{45.32} & 47.42 & \textbf{45.32}  \\
    Zhang2019Theoretically \cite{zhang2019theoretically} \dag & 55.47 & 54.21 & 54.39 & 53.45 & 53.43     & 54.23 & \textbf{53.41} \\
    %\midrule 
    Wu2020Adversarial \cite{wu2020adversarial}         & 59.05 & 56.93 & 57.02 & 56.47 & 56.44          & 56.94 & \textbf{56.42}\\
    Sehwag2021Proxy\_R18 \cite{sehwag2021robust}       & 58.68 & 57.22 & 57.89 & 56.06 & \textbf{56.05} & 57.21 & 56.06           \\
    Andriushchenko2020Understanding \cite{andriushchenko2020understanding} & 47.14 & 46.62 & 47.62 & 44.56 & 44.53 & 46.62 & \textbf{44.50} \\
    Dai2021Parameterizing \cite{dai2021parameterizing}  & 63.98 & 63.23 & 63.83 & 61.80 & \textbf{61.76} & 63.23 & 61.77           \\
    Gowal2021Improving\_28\_10\_ddpm\_100m \cite{gowal2021improving}     & 65.79 & 65.20 & 65.76 & 63.86 & 63.85          & 65.20 & \textbf{63.84}  \\
    Huang2021Exploring\_ema \cite{huang2021exploring}        & 64.95 & 64.15 & 64.64 & 63.09 & \textbf{63.03}          & 64.12 & 63.06  \\
    Zhang2020Geometry \cite{zhang2020geometry}               & 66.67 & 60.40 & 60.59 & 59.78 & \textbf{59.69} & 60.37 & \textbf{59.69} \\
    Rade2021Helper\_R18\_extra \cite{rade2021helperbased}    & 61.48 & 58.51 & 58.56 & 57.77 & \textbf{57.74} & 58.51 & \textbf{57.74}  \\
    Addepalli2021Towards\_RN18 \cite{addepalli2021towards}   & 56.00 & 51.88 & 51.97 & 51.45 & 51.43          & 51.86 & \textbf{51.41}  \\
    Sehwag2020Hydra \cite{sehwag2020hydra}                   & 59.86 & 58.41 & 58.57 & 57.66 & \textbf{57.61} & 58.40 & \textbf{57.61}  \\
    \bottomrule
    \end{tabular}
\vspace{0.2cm}
\caption{Comparing single-loss PGD with the multi-stage variant of PGD (with $K=2,3$). PGD starts from the clean point (no added noise). The experiments are executed for $T=100$ with no restarts. Each entry reports the robust accuracy of each classifier for the given method. (\dag): Attacked with $\epsilon=0.031$.}
\label{table:t100its}
\end{table*}
